Loosely-Stabilizing Phase Clocks and the Adaptive Majority Problem

We present a loosely-stabilizing phase clock for population protocols. In the population model we are given a system of $n$ identical agents which interact in a sequence of randomly chosen pairs. Our phase clock is leaderless and it requires $O(\log n)$ states. It runs forever and is, at any point of time, in a synchronous state w.h.p. When started in an arbitrary configuration, it recovers rapidly and enters a synchronous configuration within $O(n\log n)$ interactions w.h.p. Once the clock is synchronized, it stays in a synchronous configuration for at least poly $n$ parallel time w.h.p. We use our clock to design a loosely-stabilizing protocol that solves the comparison problem introduced by Alistarh et al., 2021. In this problem, a subset of agents has at any time either $A$ or $B$ as input. The goal is to keep track which of the two opinions is (momentarily) the majority. We show that if the majority has a support of at least $\Omega(\log n)$ agents and a sufficiently large bias is present, then the protocol converges to a correct output within $O(n\log n)$ interactions and stays in a correct configuration for poly $n$ interactions, w.h.p.

==> removed-text.tex <==
% Note that there are two different ways for an agent $u$ to leave $I_{gather}$.
% Either it crosses $I_{gather}$ entirely by incrementing $\Clock u$ $(6+2\cdot\sqrt{10+2})\cdot \tau$ times.
% This requires $u$ to interact only with agents in $I_{gather}$ in a row (\cref{rule:2}).
% If it interacts with an agent in $I_{work}$ it has to start over again (\cref{rule:4}).
% This slows down the faster agents in $I_{gather}$ until a large fraction of agents is in that interval.
% The second possibility is to interact with an agent $v\in I_{launch}$ (\cref{rule:3}).


%. This holds since agents reset as soon as they interact with an agent in $I_{work}$ and they can leave $I_{gather}$ only after 
%crossing the whole interval (note that agents can not hop since $I_{gather}$ is empty.$


%We will show that the combination of \cref{rule:3} and \cref{rule:4} excludes the possibility of a steady state, where agents continu 
%Recall that agents have two ways to leave $I_{gather}$.
%An agent can enter $I_{launch}$ by crossing the complete interval $I_{gather}$.
%We will show that \whp this only happens when there are at least $0.9 \cdot n$ agents in $I_{gather}$.
%Otherwise, agents can only leave $I_{gather}$ by hopping.
%But since all agents in $I_{launch}$ step forward over time, we will show that eventually there is no agent left in $I_{launch}$ to hop on.
%Then, all agents in $I_{gather}$ are stuck until there are at least $0.9 \cdot n$.
%Once, we have reached a configuration where $0.9 \cdot n $ agents are in $I_{gather}$ and no agent is in $I_{launch}$, i.e., $0.1 \cdot  n$ agents in $I_{work}$, we are almost done.
%The $0.9 \cdot n$ agents behave identical to the synchronous case.
%The remaining $0.1 \cdot n$ agents reset with probability at least $0.9$ once they enter $I_{gather}$.



From 41-maintenance:


%0 Here we  have to bound the maximum distance between the states of any pair of agents for all interactions in $[t,t'].$
Let $\Delta_{\iota} = \max_{u,v} |X_u(\iota)-X_v(\iota)|$ for all pairs of agents $u,v$ and for $\iota \in \intcc{0,t'}$.

- Using lemma 3 to bound $\Delta$.\\
- Union bound over $o(n^2)$ interactions.\\
- In the first part, we showed that agents do not hop and by definition agents do not reset before they reach $I_{gather}$.\\
- Let $t+t_u$ be the time after $t$ when $u$ enters $I_{gather}$. \\

\ctodo{Maximum der Differenzen ohne resetten betrachten, mit resetten kleiner}

- Then $\Clock{u}(t+t_u) = \Clock{u}(t) + X_u(t_u)$ for agent $u$ and 
$\Clock{u}(t+\iota) \leq \Clock{u}(t+t_u) + X_u(\iota-t_u)$ for $\iota \in \intcc{t_u,t'}$.\\
- Assuming it does not hop, we can bound the distance between any two agents $u,v$ as follows:\\
W.l.o.g. assume that $t_u < t_v$.
If $\iota \leq t_u$:
\begin{align*}
    & \big| \Clock{u}(t+\iota) - \Clock{v}(t+\iota) \big|\\
    & = \big| \Clock{u}(t) + X_{u,\iota} - (\Clock{v}(t) + X_{v,\iota}) \big| \\
    & \leq \big| \Clock{u}(t) - \Clock{v}(t) \big| + \big| X_{u,\iota} - X_{v,\iota} \big| \\
    & < |I_{launch}| + \Delta_{\iota} < |I_{gather}|.
\end{align*}
If $t_u < \iota \leq t_v$:
\begin{align*}
    & \big| \Clock{u}(t+\iota) - \Clock{v}(t+\iota) \big| \\
    & \leq \big| \Clock{u}(t+t_u) +  X_{u,\iota-t_u} - (\Clock{v}(t) + X_{v,\iota}) \big|\\
    & = \big| \Clock{u}(t) + X_{u,t_u} + X_{u,\iota-t_u} - (\Clock{v}(t) + X_{v,\iota}) \big|\\
    & \leq \big| \Clock{u}(t) - \Clock{v}(t) \big| + \big| X_{u,t_u} + X_{u,\iota-t_u} - X_{v,t_u-\iota} \big| \\
    & \leq \big| \Clock{u}(t) - \Clock{v}(t) \big| + \big| X_{u,\iota} - X_{v,t_u-\iota} \big| \\
    & < |I_{launch}| + \delta_{\iota} < |I_{gather}|.
\end{align*}
If $\iota > t_v$, $\Clock{u}{t+\iota}, \Clock{v}{t+\iota} \in I_{gather}$, hence $|\Clock{u}(t+\iota) - \Clock{v}(t+\iota)| < |I_{gather}|$.
Thus, all configurations are synchronous.

% Now we assume that $\upvarepsilon$ holds, but \cref{lem:launch->gather:2} does not.
% Then there must be a $\iota \leq t'$ where for the first time $|\Clock{u}(t+\iota) - \Clock{v}(t+\iota)| \geq |I_{launch}| + |I_{gather}|$ for some agents $u$ and $v$.
% Let $u_{\iota}$ be the agent where $\Clock{u_{\iota}}(t+\iota)$ is the maximum among all agents' states and
% let $v_{\iota}$ be the agent where $\Clock{v_{\iota}}(t+\iota)$ is the minimum among all agents' states.
% We have already shown that $\upvarepsilon$ implies that there is no interaction between agents in $I_{launch}$ and $I_{gather}$ and no agent reaches $I_{launch}$ again after leaving it.
% Therefore, we distinguish the following cases:
% \begin{enumerate}
%     \item $(\Clock{u_{\iota}}(t+\iota),\Clock{v_{\iota}}(t+\iota)) \in I_{gather}^2$: Trivially, $|\Clock{u}(t+\iota) - \Clock{v}(t+\iota)| < |I_{gather}|$.
%     \item $(\Clock{u_{\iota}}(t+\iota),\Clock{v_{\iota}}(t+\iota)) \in (I_{launch} \cup I_{work})^2$:
%     While agents are not in $I_{gather}$, they can only make a step forward.
%     Thus, $|\Clock{u}(t+\iota) - \Clock{v}(t+\iota)| = |\Clock{u}(t) + X_{u_{\iota},\iota} - (\Clock{v}(t) + X_{v_{\iota},\iota})| 
%     \leq |\Clock{u}(t) - \Clock{v}(t)| + |X_{u_{\iota},\iota} - X_{v_{\iota},\iota}| < |I_{launch}| + \Delta_{\iota} < |I_{gather}|$.    
%     \item $(\Clock{u_{\iota}}(t+\iota),\Clock{v_{\iota}}(t+\iota)) \in I_{gather} \times I_{work}$: This is identical to the case before, except that $\Clock{u}(t+\iota) \leq \Clock{u}(t) + X_{u_{\iota},\iota}$.        
% \end{enumerate}
% All cases are in contradiction to $|\Clock{u}(t+\iota) - \Clock{v}(t+\iota)| \geq |I_{launch}| + |I_{gather}|$.

This shows that the lemma holds at least with $\Prob{\upvarepsilon} = 1 - n^{-(c+1)}/2$.



























%Together, the two conditions result in the following behaviour of the phase clock.
%Assume that some agent $u$ receives a signal to start a new phase at some time $t$.
%Then the first condition ensures that there is a \emph{burst} of signals: all other agents also receive a signal within $\tau \cdot n$ interactions.
%Now the second condition ensures that there is an \emph{overlap} of agents' phases: between every two bursts, there is a time interval of length $w \cdot \tau \cdot n$ in which no agent receives a signal.


%in a time interval of length $w \cdot \tau \cdot n$ between two bursts.
%if an agent $u$ receives a signal $t$, there are at least $(w+1) \cdot \tau \cdot n$ 
%Together with the second condition it follows that
%there is an overlap of length at least $w \cdot \tau \cdot n$ %interactions during which no agent gets a signal.
%burst, overlap

%once all agents have started a new phase, there is an overlap of length at least $w \cdot \tau \cdot n$ interactions during which no agent gets a signal.
%each agent $v$ receives two consecutive signals at times $t_v$ and $t_v'$ such that $|min(t,t_v) - max(t',t_v')| \geq w \cdot n$.

%Assume agent $u$ receives a signal at time $t$
%We call this set of interactions a \emph{phase}.
%
%\item there are at least $w \cdot \tau \cdot n$ consecutive interactions where no agent receives a signal.


%Assume that agent $u_i$ receives a signal in interaction $t_1(u_i)$ and $t_2(u_i)$ but not in any interaction $t'$ with $t_1(u_i)< t'< t_2(u_i)$.
%Then
%\begin{itemize}
%\item For every agent $u_j$ there exists a interactions $t_1(u_j)$ and $t_2(u_j)$ with $|t_1(u_j)-t_1(u_i)|\le \tau n $ and $|t_2(u_j)-t_2(u_i)|\le \tau n$.
% \item $\min_j\{t_{2}(u_j)\} - \max_k\{t_{1}(u_k)\} \geq w \cdot \tau \cdot n$.
%\end{itemize}
%The first condition ensures that all agents start a new phase within $\tau n$ interactions.
%The second condition ensures that there is an overlap of $O(n \cdot w \cdot \tau)$ interactions  between the corresponding phases for all agents.

% Phase clocks are used to synchronize population protocols (\cite{}). 
% Phase clocks are simple counters $[0,\ldots Q-1]$ (modulo $Q$). 
% The counter of agent $u$ is called $\Clock u$.
% Whenever $\Clock u$ crosses zero agent $u$ receives a \emph{signal}.
% These signals can be used to divide the time into phases of
% $O(n\log n)$ interactions each.
% A set of counters define a synchronized $(\tau,w)$-phase clock if the following holds.
% Assume that agent $u_i$ receives a signal in interaction $t_1(u_i)$ and $t_2(u_i)$ but not in any interaction $t'$ with $t_1(u_i)< t'< t_2(u_i)$. Then
% \begin{itemize}
% \item $t_2(u_i)-t_1(u_i)=O(n\log n)$
% \item For every agent $u_j$ there exists a interactions $t_1(u_j)$ and $t_2(u_j)$ with $|t_1(u_j)-t_1(u_i)|\le \tau n $ and $|t_2(u_j)-t_2(u_i)|\le \tau n$.
%  \item $\min_j\{t_{2}(u_j)\} - \max_k\{t_{1}(u_k)\} \geq w \cdot n$. \ctodo{Siehe Anmerkung unten.}
% \end{itemize}
% The first condition ensures that a phase consists of $O(n\log n)$ interactions.
% The second condition ensures that all agents start a new phase within $\tau n$ interactions.
% The third condition ensures that there is an overlap of $O(n\log n)$ interactions  between the corresponding phases for all agents.
% \ctodo{Bisher sagt die Definition $w \cdot n$. Entweder der Overlap ist $w \cdot \tau \cdot n$(dann ist $w$ konstant, so wie bisher in der Definition unserer Uhr), oder wir schreiben $w = O(\log n)$. Dann muss in der Länge der Uhr $w$ durch $w/\tau$ ersetzt werden.}












from 41-maintenance:

{
\color{red}

Due to the hopping the clock counters of the agents in $I_{launch}$ are highly correlated.
Our main observation is the following:
for every agent $u$ the final state is determined by the clock increments made by several others agents $u_1, u_2\ldots$ and its own increments, and in every time step there is exactly one agent whose clock increments determine the progress of agent $u$.
Thus, we can bound the final state $u$ by a sum of random variables counting the clock increments of $u$ and $u_1, u_2,\ldots$ in the corresponding time intervals. 

In the following we assume that $u_i$ is the $i$-th agent to enter $I_{launch}$.
Agent $u_1$ enters $I_{launch}$ at time $t_0 = 0$ by increasing its counter (modulo $|Q|$) to $0$.
For the remaining agents we define so-called \emph{hopping events}. 
A hopping event is a triple $(t_i,i,j_i)$ where $t_i$ is the time when agent $u_i$ enters $I_{launch}$.
If $u_i$ enters $I_{launch}$ by increasing its clock counter we set $j_i=i$.
Otherwise $u_i$ enters $I_{launch}$ by hopping onto another agent $u_k$ with $k<i$.
In that case we set $j_i=k$.
We can now assign every agent a \emph{hopping sequence}:
The first entry of the hopping sequence of $u_i$ is $(t_i,i,j_i)$.
If $j_i\neq i$ then agent $u_i$ inherits the whole hopping sequence of agent $u_{j_i}$.
Hence, the hopping sequence of agent $u_i$ is a sequence of hopping events where the last entry belongs to an agent which entered $I_{launch}$ on its own by increasing its clock counter.

%From the result by \textcite{} (see Lemma ...) it follows that the height of a broadcast tree is 
WE MIGHT NEED A BOUND ON THE LENGTH OF A HOPPING SEQUENCE.

Consider a fixed hopping sequence $S = (t_1,i,j_1), (t_2,j_1,j_2), (t_3, j_2, j_3), \dots, (t_{k},i_{k-1},j_k)$ for agent $u_i$ of length {\color{red}$k \leq 10\log n$}.
Then $t_1>t_2> \cdots >t_{k-1}$ and $u_i$ hopped onto agent $u_{j_1}$ at time $t_1$, $u_{j_i}$ onto agent $u_{j_2}$ at time $t_2$, and so on.
We define the random variables $Z_1, \dots, Z_k$ such that $Z_i$ denotes the number of interactions initiated by agent $u_{j_i}$ in the time interval $[t_{i-1}, t_i]$,
and we define $Z_{k+1}$ as the number of interactions initiated by agent $u_i$ in the time interval $[t_1, \tilde{t}]$.
%Note that no two intervals $[t_{i}, t_{i+1}]$ overlap.
%Hence the random variables $Z_{i}$ are mutually independent.
Then we have for a fixed hopping sequence $S$
\begin{align*}
    \Clock{u_i}(\tilde{t}) \leq \min \left\{\tau-1, \sum_{i=1}^{k+1} Z_{i} \right\}.
\end{align*}
Note that $\Clock{u_i}(\tilde{t})=\tau-1$ means that the agent is in state $\Stop$.
Hence, we can express the probability of an agent $u$ reaching state $\Stop$ as
\[
\Prob{\Clock{u_i}(\tilde{t}) = \Stop | S} \leq \Prob{\sum_{i=1}^{k+1} Z_{i} \ge \tau-1 | S}. % \le \Prob{ Z_u[t'',t''+\tilde{t}] \ge \tau-1} .
\]
Recall that we have conditioned on a fixed hopping sequence $S$ for agent $u_i$.
Therefore we have to be careful when we bound $\sum_{i=1}^{k+1} Z_{i}$:
at any time, the hopping sequence $S$ rules out that certain interactions occur.
(For example, agent $u_i$ cannot initiate an interaction with agent $u_1$ before time $t_i$ since the hopping sequence rules out that $u_i$ enters $I_{launch}$ before time $t_i$.)

This means in order to bound $Z_{i}$ we must first bound the probability space $\Omega_{S}$.
That is, we give a coarse bound on the number of interactions that are possible under $S$ that holds for any point in time.
To do so, we only consider interactions where either both agents are in $I_{gather}$ or both agents are in $I_{launch}$.
Additionally, we exclude all interactions where one of the agents also occurs in the hopping sequence $S$.
%The resulting set $\tilde{\Omega}$ of interactions has the following property:
%Whenever an interaction $(u_i, v)$ occurs with positive probability, all interactions from $\tilde{\Omega}$ have the same probability.
%
%
%
%we first explicitly exclude all pairs of agents $(u,v)$ where $u \in I_{gather}$ and $v \in I_{launch}$.
%Then we exclude all interactions of agents $(u,v)$ where both $u,v \in I_{gather}$ and $u \in S$.
%
%To do so, we only consider the following (subset of) interactions that do not conflict $S$.
%
%To do so, we explicitly exclude all interactions that can possibly interact with $S$.
%These are all interactions where an agent mentioned in the hopping sequence 
%
%We only consider interactions where either both agents are in $I_{gather}$ or both agents are in $I_{launch}$, and we explicitly exclude interactions where one of the agents is part of the hopping sequence.
We observe that at each time step of the process there are at least $(n/2 - k)^2  $ such pairs of agents.
%In order to bound the random variables $Z_{i}$ we discard in each time step those interactions where the initiator is in $I_{gather}$ and the responder is in $I_{launch}$ from the underlying probability space $\Omega_{S}$.
But then the probability space $\Omega_{S}$ still contains at least $|\Omega_{S}| \geq ...$ interactions (the minimum is attained if half of the agents are in $I_{gather}$ and $I_{launch}$ each).
It follows that in each time step of the interval $[t_{i}, t_{i+1}]$ the random variable $Z_{i}$ is incremented with probability at most $(n-1) / |\Omega_{S}| \leq ...$.
Hence, we can bound the sum independently of $S$ (but conditioned on $k \geq ...$) by a binomially distributed random variable $Z(\tilde{t}) \sim \BinDistr(\tilde{t}, 2 / (n-2))$.
We get
\[
\Prob{\sum_{i=1}^{k+1} Z_{i} \ge \tau-1 | S} \le \Prob{ Z(\tilde{t}) \ge \tau-1 | S} = \Prob{ Z(\tilde{t}) \ge \tau-1} \leq n^{-c+4} .
\]
The last inequality follows from Chernoff bounds \cref{thm:chernoff-bounds} and the statement (for the simplified process) then follows from a union bound over all agents.

It is now straightforward to couple the actual phase clock process with the simplified process.
Assume that we start both processes at time $t'$ when exactly one agent is in state $0$.
In the simplified process no agent reaches state $\tau$ \whp.
This means, however, that \whp the simplified process and the actual phase clock process do not deviate.
In particular, no agent reaches the beginning of $I_{work}$ in $t''$ whatever TODO many interactions.
Thus, the configuration $C_{t'}$ is \whp a homogeneous launching configuration.

%We apply Chernoff bounds to $Z(\tilde{t})$ and obtain
%\[
%\Prob{\sum_{i=1}^{k+1} Z_{i} \ge \tau-1} \geq 1 - 1/n^{42}.
%\]
%The statement follows from a union bound over all agents.

============ =============
Assume agents leave gather in order 1,...,n
Induction hypothesis: $\Prob{\Clock{u_i}(t') \geq k} \leq \Prob{\Clock{u_1}(t') \geq k}$

=========================
% \begin{align*}
%     &\Prob{\Clock{u_i}(t') \geq k}\\
%     &=\sum_{j<i} \sum_{(t,p) \in \intcc{0,t'} \times \intcc{0,k}} \Prob{\Clock{u_i}(t') \geq k | \Clock{u_j}(t) = p \land i \text{ hops on }j} \cdot \Prob{\Clock{u_j}(t) = p} \cdot \Prob{i \text{ hops on }j}\\
%     &=\sum_{j<i} \sum_{(t,p) \in \intcc{0,t'} \times \intcc{0,k}} \Prob{Z_i(t+1,t') \geq k-p | \Clock{u_j}(t) = p \land i \text{ hops on }j} \cdot \Prob{\Clock{u_j}(t) = p} \cdot \Prob{i \text{ hops on }j}\\
%     &=\sum_{j<i} \sum_{(t,p) \in \intcc{0,t'} \times \intcc{0,k}} \Prob{Z_j(t+1,t') \geq k-p | \Clock{u_j}(t) = p \land i \text{ hops on }j} \cdot \Prob{\Clock{u_j}(t) = p} \cdot \Prob{i \text{ hops on }j}\\
%     &<\sum_{j<i} \Prob{\Clock{u_j}(t') \geq k} \cdot \Prob{i \text{ hops on }j} =^{IV} \Prob{\Clock{u_1}(t') \geq k}
% \end{align*}


========================

The random variable $Z_u[t'',t''+\tilde{t}]$ denotes the number of interactions of an agent $u$ in the time interval $[t'', t'' + \tilde{t}]$.


Observe that $Z_u[t'',t''+\tilde{t}]$ is majorized by a binomial distribution $X \sim \BinDistr(\tilde{t},p)$.
We can bound $p$ as follows:
There are $n^2$ possible interactions in total.
Since we condition on the history of hopping events, we discard every interaction that is a pair of an initiator in $I_{launch}$ and a responder in $I_{gather}$ - at most $n^2/4$.
Thus, per agent in $I_{launch}$ there are $n$ interactions where this agent is the initiator among at least $3/4\cdot n^2$ interactions from which we sample uniformly at random, i.e., $p \leq 4/(3\cdot n)$.

For $\tilde{t}_2=0.5 \cdot \tau \cdot n$, we have $\Ex{X} = (2/3) \cdot \tau$.
We use \cref{lemma:chernoff_poisson_trials} for a bound with high probability.
\begin{align*}
    &\Prob{\Clock{u_i}(t''+\tilde{t}) = \Stop}
    \leq \sum_{s \in \Omega} \Prob{\Clock{u_i}(t''+\tilde{t}) = \Stop | s} \cdot \Prob{s}\\
    &\leq \sum_{s \in \Omega} \Prob{X \geq \tau-1} \cdot \Prob{s}
    \leq \Prob{X_{t'_2} \geq \tau} \cdot \sum_{s \in \Omega} \Prob{s}
    =\Prob{X_{t_2'} \geq \tau}  \leq n^{-\frac{\tau}{12 \cdot \ln n}} = n^{-(c+4)}.
\end{align*}
By a union bound, this holds for all agents with probability at least $1-n^{-(c+3)}$.

The probability of all agents having a non-empty history (i.e., reaching $I_{launch}$) and none reaching state $\tau$ within $0.5 \cdot \tau \cdot n$ interactions is at least $1 - n^{-(c+2)} - n^{-(c+3)} \geq 1 - n^{-(c+1)}/2$.

Finally, we couple our process with the simplified process.
Assume that we start both processes at time $t'_1$ where exactly one agent is in state $0$.
We have just proven that \whp no agent in the simplified process reaches state $\tau$ (the beginning of $I_{work}$) within the next $t'_2$ interactions.
Therefore, under the same set of interactions neither does any agent in the original process and thus both processes behave identically.
Thus, for $t' = t'_1 +t'_2$, the configuration $C_{t'}$ is \whp a homogeneous launching configuration.

